Learning Generalizable Latent Representations for Novel Degradations in Super Resolution

Typical methods for blind image super-resolution (SR) focus on dealing with unknown degradations by directly estimating them or learning the degradation representations in a latent space. A potential limitation of these methods is that they assume the unknown degradations can be simulated by the integration of various handcrafted degradations (e.g., bicubic downsampling), which is not necessarily true. The real-world degradations can be beyond the simulation scope by the handcrafted degradations, which are referred to as novel degradations. In this work, we propose to learn a latent representation space for degradations, which can be generalized from handcrafted (base) degradations to novel degradations. The obtained representations for a novel degradation in this latent space are then leveraged to generate degraded images consistent with the novel degradation to compose paired training data for SR model. Furthermore, we perform variational inference to match the posterior of degradations in latent representation space with a prior distribution (e.g., Gaussian distribution). Consequently, we are able to sample more high-quality representations for a novel degradation to augment the training data for SR model. We conduct extensive experiments on both synthetic and real-world datasets to validate the effectiveness and advantages of our method for blind super-resolution with novel degradations.

==> table1.tex <==


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\caption{SR performance of our method with and without sampling. The results of Bulat \textit{et al.} without sampling are provided for reference.}
\vspace{-5pt}
\renewcommand\arraystretch{1.1}
\resizebox{1\linewidth}{!}{
    \begin{tabular}{l|ccc|ccc}
        \toprule
        \multirow{2}{*}{Method} & 
        \multicolumn{3}{c|}{AIM 2019 dataset}  & 
        \multicolumn{3}{c}{NTIRE 2020 dataset} \\
         & PSNR$\uparrow$  & SSIM$\uparrow$  & LPIPS $\downarrow$ & PSNR$\uparrow$  & SSIM$\uparrow$  & LPIPS$\downarrow$     \\
        \midrule
Our (w/o sampling) & 22.08 & 0.675 & 0.187 & 23.76     & 0.658   & 0.127    \\
Ours (with sampling)  & \textbf{22.10}  & \textbf{0.688} & \textbf{0.175}              & \textbf{23.85}     & \textbf{0.670}    & \textbf{0.120}    \\
\bottomrule
    \end{tabular}}
\vspace{-5pt}
\label{tab:sample}
\end{table}

\begin{comment}
\begin{table*}[t]
\caption{SR performance of our method with and without sampling.}
\vspace{-5pt}
\renewcommand\arraystretch{1.1}
\resizebox{1\linewidth}{!}{
    \begin{tabular}{l|ccc|ccc|ccc|ccc}
        \toprule
              \multirow{3}{*}{Method} & 
        \multirow{3}{*}{Scale} &
        \multicolumn{6}{c|}{Synthetic data}&
        \multicolumn{6}{c}{Real-world data}\\
        & &\multicolumn{3}{c|}{Camera sensor noise}  & 
        \multicolumn{3}{c|}{Jpeg compression} &
        \multicolumn{3}{c|}{AIM 2019 dataset}  & 
        \multicolumn{3}{c}{NTIRE 2020 dataset}\\
          & & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$  & PSNR$\uparrow$        & SSIM$\uparrow$      & LPIPS$\downarrow$ & PSNR$\uparrow$        & SSIM$\uparrow$      & LPIPS$\downarrow$& PSNR$\uparrow$        & SSIM$\uparrow$      & LPIPS$\downarrow$\\
        \midrule
Bulat \textit{et al.}~\cite{DegradationGAN} & 28.68 &0.526 & 0.474 & 28.40 & 0.351 & 0.708    \\
Our (w/o sampling) & 28.79 & 0.664 & 0.478 & 28.72     & 0.437   & 0.697    \\
Ours (with sampling)  & \textbf{28.88}  & \textbf{0.688} & \textbf{0.448}              & \textbf{28.81}     & \textbf{0.465}    & \textbf{0.642}    \\
\bottomrule
    \end{tabular}}
\vspace{-5pt}
\label{tab:sample}
\end{table*}
\end{comment}

